Comparative Benchmarking of Causal Discovery Techniques

In this paper we present a comprehensive view of prominent causal discovery algorithms, categorized into two main categories (1) assuming acyclic and no latent variables, and (2) allowing both cycles and latent variables, along with experimental results comparing them from three perspectives: (a) structural accuracy, (b) standard predictive accuracy, and (c) accuracy of counterfactual inference. For (b) and (c) we train causal Bayesian networks with structures as predicted by each causal discovery technique to carry out counterfactual or standard predictive inference. We compare causal algorithms on two pub- licly available and one simulated datasets having different sample sizes: small, medium and large. Experiments show that structural accuracy of a technique does not necessarily correlate with higher accuracy of inferencing tasks. Fur- ther, surveyed structure learning algorithms do not perform well in terms of structural accuracy in case of datasets having large number of variables.

==> Sections/data_description.tex <==
\textbf{Data Description: }
We use real datasets for providing a comprehensive evaluation of all the available causal structure learning algorithms. 

\textbf{\textit{Sachs :}} We use the Sachs dataset which consists of single cell expression profiles of 11 phosphorylated proteins involved in a signaling pathway of human primary T cells. 

\textbf{\textit{DREAM4 :}} We use the DREAM4 10-node and 100-node in-silico network reconstruction challenge, which is a commonly used benchmark data for network inference algorithms. They provide five networks each for both 10 and 100-node respectively with different structures, all chosen to reflect common topological properties of real gene regulatory networks in E. coli or S. cerevisiae, which include feedback loops. Stochastic differential equations and a realistic noise model of microarray data sets are used to generate expression data from each network. 


==> Sections/experiments-1.tex <==
\subsection{Data Description:}

Comprehensive evaluations of causal structure learning algorithms is carried out using two real datasets and one simulated dataset.

\textbf{DREAM4 dataset:} Data from \textit{in-silico} gene regulatory network~\cite{greenfield2010dream4} was used for benchmarking network inferencing algorithms. DREAM4 datasets were generated from five networks each for both 10 and 100 nodes respectively with different structures which include feedback loops.
For $10-$node DREAM4 networks, 1 wild type and 10 multifactorial perturbation data samples are jointly considered as \textit{DREAM4$\_$10 observational} dataset. \textit{DREAM4$\_$10 intervention} datasets consists of 20 intervention samples, which consist of one knockout and one knockdown per gene. For $100-$node DREAM4 networks, 201 samples containing 1 wildtype , 100 knockdown and 100 knockout instances are considered as \textit{DREAM4$\_$100 observational datasets}. 

\textbf{Sachs dataset:} Sachs dataset~\cite{sachs2005causal} consists of data collected after general perturbation, which relied on simultaneous measurement of single cell expression profiles of 11 phosphorylated proteins involved in a signaling pathway of human primary T cells. This data is termed as \textit{Sachs observational} dataset in this paper. Dataset was also collected after inhibitory interventions on specific set of molecules. This dataset is named as \textit{Sachs intervention} dataset and consists of 8142 samples obtained by inhibitory cues on defined set of molecules.   

\textbf{Simulated dataset:} Data is generated randomly from 10-node Gaussian Bayesian network in \cite{cho2016reconstructing}. Each edge weight is uniformly sampled from $(-1,-.25) \cup (.25,1)$. Base level of each node is randomly sampled from uniform distribution $\cup(50,500)$ and noise-level for each node is uniformly sampled from $\cup(5,100)$. 10,000 data samples are generated from this model and termed as \textit{Simulated observational} dataset. Knock-out intervention data is also simulated from the same model by knocking out each node sequentially to generate 1000 interventional samples corresponding to each node. The data generated by such inhibitory cues is named as \textit{Simulated intervention} dataset.


%%\linebreak
%\paragraph{} We use the pcalg-R implementation for estimating the equivalence class of a directed acyclic graph (DAG) from data.
%
%We vary the alpha,significance level from (0.0 to 1.0)in increments of 0.01 for the individual conditional independence tests to find the best causal graph structure.
%
%\subsection{\textbf{Deciding Optimal Significance Level:}}  
%For deciding the optimal level of significance level we calculate Precision, Recall , F-Score and AUC(Area under the receiver operating characteristic curve) for finding the most accurate underlying causal structure obtained. Our metric for evaluation is similar as in the DREAM4 challenge.
%
%\textbf{Definitions } 
%\linebreak
%\textit{True Positive:} Count of the number of edges, taking into account their orientation, that are present both in the original structure and the learned structure
%
%\textit{True Negative:} Count of the number of edges,taking into account their orientation,that are not present in original structure and the learned structure 
%
%\textit{False Positive:} Count of the number of edges, taking into account their orientation,that are  present in learned structure but not in the original structure  
%
%\textit{False Negative:} Count of the number of edges,  taking into account their orientation, that are not present in the learned structure but are present in the original structure.
%\textit{Precision:}
%\textit{Recall:}
%\textit{F-Score:}
%\textit{Area under the ROC:}

\subsection{Implementation aspects of causal structural algorithms}

Structure learning algorithms are broadly classified into five major categories, as described in section~\ref{section:estimating_structures}. Implementation details of each algorithm is discussed below:

\textbf{On observational data}
 
PC : 
We estimate the equivalence class of DAG from observational data, using PC-algorithm. We use pcalg-R implementation where conditional independence of pair of edges given conditioning set $S$ assumes the data to be from multivariate normal distribution and uses the concept that zero partial correlation is equivalent to conditional independence for determining skeleton of the graph. For varying values of significance levels (0 to 1 in steps of 0.01) of conditional independence tests, different CPDAGs can be obtained.

GES :
We estimate the observational essential graph representing the Markov equivalence class of a DAG using the greedy equivalence search (GES) algorithm of \cite{chickering2002optimal} implemented in pcalg-R. We use $l$0-penalized Gaussian maximum likelihood estimator for scoring the candidate graph networks. 

MMHC :
We use the \cite{tsamardinos2006max} implementation of the Max-Min Hill Climbing Algorithm given in the bnlearn-R package. We use the BIC criterion as the scoring algorithm and vary  the target nominal type I error rate of the conditional independence test for finding the best possible structure based on F-Score as the measure for correctness.

GBN: 
We use the implementation of GBN given in \cite{cho2016reconstructing}. The output of GBN based algorithm is the graph obtained by model averaging of the set of sampled graph structures drawn from the posterior distribution, where posterior represents how strong is each candidate graph structure to the underlying model given the data. Edge weights of the averaged, weighted resultant graph structure are normalized between 0 to 1 and thresholded at different levels to obtain different CPDAGs corresponding to each threshold level.

\textbf{On observational and intervention data} We apply GIES and GBN algorithms to learn causal structure using both observational as well as intervention data.

GIES : 
We use \cite{hauser2012characterization} implementation given in pcalg-R for estimating markov equivalence of a DAG using GIES algorithm. $l$0-penalized Gaussian maximum likelihood estimator is used for scoring candidate causal graph structures learned jointly from interventional and observational data.

GBN : We use same implementation as discussed above except that both observational and interventional data is used in this case.

\textbf{Assuming hidden variables:} Use of non-experimental data for discovery of causal relations is usually faced with the problem of latent or confounding variable, where confounding factors affecting measured variables may not have been measured. 
We discuss the implementation specifics of algorithms which take into account hidden variable assumption in this section. 

FCI :
The first part of the FCI algorithm is analogous to the PC algorithm. FCI algorithm gives a resultant PAG.\cite{richardson1996discovery}  For orienting the possible undetermined edge marks (o) \cite{zhang2008causal} \cite{zhang2008completeness} orientation rules are used. 

FCI+ :
FCI Plus is a variation of the Fast Causal Algorithm. We use the pcalg-R implementation for the same as given by \cite{claassen2013learning} which implements  the  method  for an independence oracle, and suggests improvements for sample/real-world data version

RFCI :
RFCI does not compute any Possible-D-SEP sets and thus does not make tests conditioning on subsets of Possible-D-SEP. This makes RFCI much faster than FCI. We use the \cite{colombo2012learning} given in pcalg-R for computation.

\textbf{Assuming cycles:} We use CCD algorithm implemented in TETRAD for learning cyclic causal structures. Causal structures corresponding to significance values varying between 0 to 1 with step-size of 0.1 are obtained.

\textbf{Active Learning:} Interventional experiments are usually costly and hence number of experiments that can be performed are limited in number. Active learning framework thus helps to choose interventions which are most informative, thus enabling design of interventional experiments subject to time/cost constraints while maximizing the use of less resources.  We explore the work of \cite{cho2016reconstructing} which uses active learning to priortize the interventions for optimal results using GBN framework. 
We use \textit{DREAM4$\_$10 observational dataset} and \textit{DREAM4$\_$10 interventional datasets}(knockout data) to prioritize 10 interventions in 3 trials of experiments. 
\subsection{Performance Metrics}
Well known causal structure learning algorithms are used for estimating causal networks. These learned networks are used for measuring effectiveness of algorithms based on two broad types of performance metrics:

\textbf{Structural efficiency based metrics} 

\textit{Structural F-score} and Area under ROC curve (\textit{AUC}) are used for measuring structural effectiveness of the algorithm. 

For the learned structure, each edge is defined as true positive, true negative, false positive, false negative based on the definitions in Figure~\ref{fig:confusion_matrix}. Structural precision, recall and false positive rate (FPR) are evaluated for varying thresholds on significance values/edge weights using eq~\ref{eq:precision}, eq~\ref{eq:recall}, eq~\ref{eq:fpr}.
\begin{equation}
  \small
   Precision = \frac{\sum_{i} Tp_{i}}{\sum_{i} Tp_{i}+\sum_{i} Fp_{i}}
   \label{eq:precision}
\end{equation}
\begin{equation}
  \small
   Recall = \frac{\sum_{i} Tp_{i}}{\sum_{i} Tp_{i}+\sum_{i} Fn_{i}}
   \label{eq:recall}
\end{equation}
\begin{equation}
  \small
  FPR = \frac{\sum_{i} Fp_{i}}{\sum_{i} tn_{i}+\sum_{i} fp_{i}}
   \label{eq:fpr}
\end{equation}

F-score is the harmonic mean of precision and recall and is computed at each threshold level. For this study, highest value of F-score is termed as \textit{structural F-score}. Area under ROC (curve plotting Recall versus fpr at different thresholds) is termed as \textit{structural AUC} and represents the overall effectiveness of causal structure learning algorithm over different levels of parameters-significance value/edge weights.
\begin{figure}[h]
\centering
\includegraphics[width = 80mm]{Figures/confusion_matrix.png}
%\vspace{6pt}
\caption{Confusion matrix defining measures classifying each edge as True positive, True negative, False positive and False negative.}
\label{fig:confusion_matrix}
%\vspace{-10pt}
\end{figure}

\textbf{Inferencing capability based metric:} Standard metric for measuring performance of causal learning algorithms involve measures like structure hamming distance, F-score, count of missing and present edges. All these measures calculate structural efficiency of structure. However, practical application of structure learning involve inferencing from the learned causal graph. Inferencing a causal network can assist in multiple practical applications involving predictions, interventional queries and counterfactual reasonong. Hence, we propose a novel measure \textit{Predictive accuracy}, which is used to measure the inferencing capability of the structure with best \textit{Structural F-score}.

For calculating \textit{predictive accuracy}, we extend selected PAG/CPDAG to DAG using \cite{dor1992simple}. If no extension is possible, DAG corresponding to the skeleton of the PDAG is taken. Having obtained DAG structure, we predict the values of each node by evidencing on remaining nodes of the learned network (using exact inferencing) and then calculate normalized root mean squared error (NRMSE) of the predicted values with respect to the actual value in the data. Averaged out NRMSE across all node of each learned network is shown in Table \ref{NRMSE}.

\subsection{\textbf{Comparison of algorithms based on structure obtained(F-Score and AUC ):} }

\textit{DREAM4 - 10 node in silico network:}

Table 1 represents the F-Score and AUC for each network obtained after applying the fore mentioned algorithms to the DREAM4 and Sachs datasets.

We found that GIES consistently outperforms GES algorithm in terms of F-Score and AUC irrespective of the variety of networks to which it was applied. Also, PC algorithm inspite of having various assumptions it at par in terms of performance with all the other available algorithms.

We also noted that the networks obtained by applying GES and GIES algorithm are much more complex in comparison to all other algorithms applied which provide a much spaser network.
\subsubsection{Performance of active learning on DREAM\_4 dataset}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{\#Nodes}} & \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}SCORE\\  (alpha)\end{tabular}}} & \multicolumn{10}{c|}{\textbf{Algorithms}}                                                                                                                                                                                                                                                                                                                                                                                                       \\ \cline{4-13} 
                                  &                                   &                                                                                    & \textit{PC}                                                 & \textit{GES} & \textit{GIES} & \textit{FCI}                                                & \textit{FCI+}                                               & \textit{RFCI}                                               & \textit{CCD}                                            & GBN              & GBNobs+int                                         & MMHC          \\ \hline
\multirow{2}{*}{10}               & \multirow{2}{*}{DREAM\_1}         & \textit{Fm}                                                                        & \begin{tabular}[c]{@{}c@{}}0.41176\\  ( 0.68 )\end{tabular} & 0.29411      & 0.35897       & \begin{tabular}[c]{@{}c@{}}0.41176\\ ( 0.11 )\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.41176\\  ( 0.11 )\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.41176\\  ( 0.11 )\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.3478\\ (0.25)\end{tabular} & 0.2857143 (0.06) & \begin{tabular}[c]{@{}l@{}}0.3846154 \\ (0.25)\end{tabular} & 0.36 (0.53)   \\ \cline{3-13} 
                                  &                                   & \textit{AUC}                                                                       & 0.55274                                                     & 0.59136      & 0.64534       & 0.26868                                                     & 0.34385                                                     & 0.34385                                                     & 0.527                                                   & 0.5606312        & 0.6677741                                                   & 0.549         \\ \hline
\multirow{2}{*}{10}               & \multirow{2}{*}{DREAM4\_2}        & \textit{Fm}                                                                        & \begin{tabular}[c]{@{}c@{}}0.45454\\  ( 0.07 )\end{tabular} & 0.28571      & 0.29411       & \begin{tabular}[c]{@{}c@{}}0.42105\\  ( 0.04 )\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.44 \\ ( 0.59 )\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0.44 \\ ( 0.59 )\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0.4242\\ (0.9)\end{tabular}  & 0.3728814 (0.28) & \begin{tabular}[c]{@{}l@{}}0.4375 \\ (0.15)\end{tabular}    & 0.3448 (0.82) \\ \cline{3-13} 
                                  &                                   & \textit{AUC}                                                                       & 0.5762                                                      & 0.56845      & 0.5788        & 0.18117                                                     & 0.30617                                                     & 0.30617                                                     & 0.572                                                   & 0.6997768        & 0.7291667                                                   & 0.5758        \\ \hline
\multirow{2}{*}{10}               & \multirow{2}{*}{DREAM4\_3}        & \textit{Fm}                                                                        & \begin{tabular}[c]{@{}c@{}}0.4375 \\ ( 0.42 )\end{tabular}  & 0.11764      & 0.17647       & \begin{tabular}[c]{@{}c@{}}0.4375 \\ ( 0.01 )\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.4375 \\ ( 0.01 )\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.4375 \\ ( 0.01 )\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.1739\\ (0.25)\end{tabular} & 0.4324324 (0.48) & \begin{tabular}[c]{@{}l@{}}0.4137931\\  (0.29)\end{tabular} & 0.4 (0.19)    \\ \cline{3-13} 
                                  &                                   & \textit{AUC}                                                                       & 0.54152                                                     & 0.46677      & 0.50830       & 0.27034                                                     & 0.33222                                                     & 0.33139                                                     & 0.4755                                                  & 0.6856312        & 0.6652824                                                   & 0.615         \\ \hline
\multirow{2}{*}{10}               & \multirow{2}{*}{DREAM4\_4}        & \textit{Fm}                                                                        & \begin{tabular}[c]{@{}c@{}}0.3265\\  ( 0.95 )\end{tabular}  & 0.1212       & 0.29411       & \begin{tabular}[c]{@{}c@{}}0.30303\\ ( 0.19 )\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.32653\\  ( 0.81 )\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.32653\\  ( 0.81 )\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.444\\ (0.9)\end{tabular}   & 0.3414634 (0.18) & \begin{tabular}[c]{@{}l@{}}0.75 \\ (0.29)\end{tabular}      & 0.2727 (0.63) \\ \cline{3-13} 
                                  &                                   & \textit{AUC}                                                                       & 0.49292                                                     & 0.47347      & 0.60035       & 0.24801                                                     & 0.3315                                                      & 0.33068                                                     & 0.509                                                   & 0.658267         & 0.801061                                                    & 0.5503        \\ \hline
\multirow{2}{*}{10}               & \multirow{2}{*}{DREAM4\_5}        & \textit{Fm}                                                                        & \begin{tabular}[c]{@{}c@{}}0.4375 \\ ( 0.84 )\end{tabular}  & 0.27778      & 0.35294       & \begin{tabular}[c]{@{}c@{}}0.46153\\  ( 0.6 )\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.4444\\  ( 0.62 )\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.4444\\  ( 0.62 )\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.4545\\ (0.85)\end{tabular} & 0.3888889 (0.29) & \begin{tabular}[c]{@{}l@{}}0.4705882 \\ (0.56)\end{tabular} & 0.33 (0.89)   \\ \cline{3-13} 
                                  &                                   & \textit{AUC}                                                                       & 0.65104                                                     & 0.60037      & 0.65909       & 0.32481                                                     & 0.38162                                                     & 0.38162                                                     & 0.5762                                                  & 0.7357955        & 0.8309659                                                   & 0.5757        \\ \hline
\multirow{2}{*}{11}               & \multirow{2}{*}{Sachs}            & \textit{Fm}                                                                        & \begin{tabular}[c]{@{}c@{}}0.45\\  (0.01)\end{tabular}      & 0.2857       & 0.1034        & \begin{tabular}[c]{@{}c@{}}0.45 \\ (0.01)\end{tabular}      & \begin{tabular}[c]{@{}c@{}}0.45\\  (0.01)\end{tabular}      & \begin{tabular}[c]{@{}c@{}}0.45\\  (0.01)\end{tabular}      & \multicolumn{1}{c|}{0.45}                               & 0.3571429 (0.01) & \begin{tabular}[c]{@{}l@{}}0.15 \\ (0.01)\end{tabular}      & 0.4137 (0.01) \\ \cline{3-13} 
                                  &                                   & \textit{AUC}                                                                       & 0.676                                                       & 0.579        & 0.403         & 0.6801                                                      & 0.6758                                                      & 0.6758                                                      & \multicolumn{1}{c|}{0.4868}                             & 0.6098512        & 0.4688164                                                   & 0.62783       \\ \hline
\end{tabular}
\caption{My caption}
\label{my-label}
\end{table*}

\textit{DREAM4 - 100 node in silico network:}

We use 201 samples as observational data and 200 samples as intervention data for the 100 node DREAM4 networks.

\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|l|}
\hline
\multirow{2}{*}{\textbf{\#Nodes}} & \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textit{\textbf{SCORE (alpha)}}} & \multicolumn{7}{c|}{\textbf{Algorithms}} \\ \cline{4-10} 
 &  &  & \textit{PC} & \textit{GES} & \textit{GIES} & \textit{FCI} & \textit{FCI+} & \textit{RFCI}  \\ \hline
\multirow{2}{*}{100} & \multirow{2}{*}{DREAM4\_1} & \textit{Fm} & \begin{tabular}[c]{@{}c@{}}0.23529\\  (0.4)\end{tabular} & 0.60869 & 0.13793 & \begin{tabular}[c]{@{}c@{}}0.15384\\ (0.3)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.15384\\ (0.3)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.15384\\ (0.3)\end{tabular} &  \\ \cline{3-10} 
 &  & \textit{AUC} & 0.57626 & 0.56845 & 0.57886 & 0.18117 & 0.30617 & 0.30617 &  \\ \hline
\multirow{2}{*}{100} & \multirow{2}{*}{DREAM4\_2} & \textit{Fm} & \begin{tabular}[c]{@{}c@{}}0.14814\\ (0.4)\end{tabular} & 0.26086 & 0.20689 & \begin{tabular}[c]{@{}c@{}}0.10526\\ (0.1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.10526\\ (0.1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.10526\\ (0.1)\end{tabular} &  \\ \cline{3-10} 
 &  & \textit{AUC} & 0.0086 & 0.58580 & 0.55209 & 0.00204 & 0.00204 & 0.00204 &  \\ \hline
\multirow{2}{*}{100} & \multirow{2}{*}{DREAM4\_3} & \textit{Fm} & \begin{tabular}[c]{@{}c@{}}0.18181 \\ (0.6)\end{tabular} & 0.09523 & 0.20689 & \begin{tabular}[c]{@{}c@{}}0.086856\\ (0.1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.086856\\ (0.1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.086856\\ (0.1)\end{tabular} &  \\ \cline{3-10} 
 &  & \textit{AUC} & 0.013278 & 0.49489 & 0.55209 & 0.00204 & 0.00204 & 0.00204 &  \\ \hline
\multirow{2}{*}{100} & \multirow{2}{*}{DREAM4\_4} & \textit{Fm} & \begin{tabular}[c]{@{}c@{}}0.17391\\ (0.2)\end{tabular} & 0.09090 & 0.06896 & \begin{tabular}[c]{@{}c@{}}0.17391\\ (0.3)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.17391\\ (0.3)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.17391\\ (0.3)\end{tabular} &  \\ \cline{3-10} 
 &  & \textit{AUC} & 0.02451 & 0.48927 & 0.44994 & 0.00612 & 0.00408 & 0.00408 &  \\ \hline
\multirow{2}{*}{100} & \multirow{2}{*}{DREAM4\_5} & \textit{Fm} & \begin{tabular}[c]{@{}c@{}}0.5 \\ (0.4)\end{tabular} & 0.32258 & 0.27778 & \begin{tabular}[c]{@{}c@{}}0.5 \\ (0.5)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.5 \\ (0.5)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.5 \\ (0.5)\end{tabular} &  \\ \cline{3-10} 
 &  & \textit{AUC} & 0.04876 & 0.62878 & 0.60037 & 0.03030 & 0.03030 & 0.03030 &  \\ \hline
\end{tabular}
\caption{F-Score and AUC values for DREAM4 100-node networks}
\label{my-label}
\end{table*}

\subsection{\textbf{Comparison of algorithms based on Predictive Accuracy:} }


\subsubsection{Performance of active learning on DREAM\_4 dataset}
   
\begin{table*}[]
\centering
\begin{tabular}{|p{5.2em}|p{4.2em}|p{4.2em}|p{4.2em}|p{4.2em}|p{4.2em}|p{4.2em}|p{5.2em}|}
\hline
 & \textit{DREAM4$\_$1} & \textit{DREAM4$\_$2} & \textit{DREAM4$\_$3} & \textit{DREAM4$\_$4} & \textit{DREAM4$\_$5} & \textit{Sachs} dataset & AVERAGE \\ \hline
PC                 & 9.01                       & 31.43                      & 32.79                      & 32.13                      & 33.15                      & 6.2       & 24.1183                   \\ \hline
GES               & 7.62                       & 8.3                        & 10.18                      & 10.43                      & 10.24                      & 6.3                  & 8.845                     \\ \hline
GBN(obs)                    & $*$                         & 8.32                       & 11.57                      & 9.91                       & 11.17                      & 6.836                  & 9.56                   \\ \hline
MMHC                   & 16.84                        & 10.12                 & 22.39                    & 16.87                       & 12.58                      & 8.78                &                         14.59 \\ \hline
GIES              & 10.45                      & 11.3                       & 12.45                      & 11.67                      & 10.24                      & 7.32                    & 10.5716                   \\ \hline
GBN(obs+int)                & 17.54                      & 7.5                        & 17.5                       & 15.18                      & 23.52                      & 6.26                     & 14.58                         \\ \hline
FCI                & 15.72                      & 10.8                       & 10.04                      & 13.08                      & 14.66                      & 6.59                   & 11.815                    \\ \hline
FCIP             & 10.53                      & 11.05                      & 10.09                      & 7.82                       & 18.63                      & 6.24                   & 10.7267                   \\ \hline
RFCI              & 15.16                      & 7.76                       & 8.09                       & 7.87                       & 16.33                      & 6.39                  & 10.2667                   \\ \hline
Active Learning             & 12.27                      & 17.37                      & 15.58                      & 11.47                      & 11.97                      & $\_$  & 13.73                                     \\ \hline
\end{tabular}
\caption{Averaged out normalized mean squared errors corresponding to real datasets. obs: stands for observational dataset and int: stands for intervention dataset. * took more than a day for execution (Results are not presented for the same). }
\label{NRMSE}

\end{table*}
We found that in terms of Predictive Accuracy GES consistently outperformed all the other algorithms with average NRMSE value of 8.845


\subsection{Relation of performance metrics with dataset size}
 

==> Sections/experimentsbackup.tex <==
In this section, we present comparitive benchmark of structure learning algorithms (discussed in section~\ref{sec:experiments}) over three datasets having different sample sizes.

\subsection{Data Description:} Comprehensive evaluations of causal structure learning algorithms is carried out using two real datasets and one simulated dataset.

\textbf{DREAM4 dataset:} Data from \textit{in-silico} gene regulatory network~\cite{greenfield2010dream4} is used for benchmarking structure learning algorithms. DREAM4 dataset are generated from five networks each for both 10 and 100 nodes respectively with different structures which include feedback loops.
For $10-$node DREAM4 networks, 1 wild type and 10 multifactorial perturbation data samples are considered as observational dataset while intervention dataset consists of 20 intervention samples, consisting of one knockout and one knockdown per gene. $100-$node DREAM4 networks consists of 201 samples containing 1 wildtype, 100 knockdown and 100 knockout instances.

\textbf{Sachs dataset:} Sachs dataset~\cite{sachs2005causal} consists of observational data collected after general perturbation, which relied on simultaneous measurement of single cell expression profiles of 11 phosphorylated proteins involved in a signaling pathway of human primary T cells. Sachs dataset contains 8142 samples obtained by inhibitory cues on defined set of molecules.   

\textbf{Simulated dataset:} Data is generated randomly from 10-node Gaussian Bayesian network in \cite{cho2016reconstructing}. Each edge weight is uniformly sampled from $(-1,-.25) \cup (.25,1)$. Base level of each node is randomly sampled from uniform distribution $\cup(50,500)$ and noise-level for each node is uniformly sampled from $\cup(5,100)$. 10,000 observational data samples are generated from this model. Knock-out intervention data is also simulated from the same model by knocking out each node sequentially to generate 1000 intervention samples per node. 


%%\linebreak
%\paragraph{} We use the pcalg-R implementation for estimating the equivalence class of a directed acyclic graph (DAG) from data.
%
%We vary the alpha,significance level from (0.0 to 1.0)in increments of 0.01 for the individual conditional independence tests to find the best causal graph structure.
%
%\subsection{\textbf{Deciding Optimal Significance Level:}}  
%For deciding the optimal level of significance level we calculate Precision, Recall , F-Score and AUC(Area under the receiver operating characteristic curve) for finding the most accurate underlying causal structure obtained. Our metric for evaluation is similar as in the DREAM4 challenge.
%
%\textbf{Definitions } 
%\linebreak
%\textit{True Positive:} Count of the number of edges, taking into account their orientation, that are present both in the original structure and the learned structure
%
%\textit{True Negative:} Count of the number of edges,taking into account their orientation,that are not present in original structure and the learned structure 
%
%\textit{False Positive:} Count of the number of edges, taking into account their orientation,that are  present in learned structure but not in the original structure  
%
%\textit{False Negative:} Count of the number of edges,  taking into account their orientation, that are not present in the learned structure but are present in the original structure.
%\textit{Precision:}
%\textit{Recall:}
%\textit{F-Score:}
%\textit{Area under the ROC:}

\subsection{Implementation aspect of causal structural algorithms}

We have broadly categorised the various causal structure learning techniques into five major classes, as described in Section~\ref{sec:estimating_structures}. From each class, we have chosen the most prevalent algorithms for which the implementation details are discussed below:

\textbf{Using observational data:} PC : To estimate the equivalence class of DAG from observational data, using PC-algorithm we use pcalg-R \cite{kalisch2010pcalg} implementation. The conditional independence of pair of edges given conditioning set $S$ assumes the data to be from multivariate normal distribution and uses Fisher Z-Score conditional independence test for determining skeleton of the graph. By varying values of significance level (0 to 1 in steps of 0.01) of conditional independence tests, different CPDAGs are obtained.

GES : Using the greedy equivalence search observational essential graph  \cite{chickering2002optimal} representing the Markov equivalence class of a DAG is estimated ,implemented in pcalg-R. We use $l$0-penalized Gaussian maximum likelihood estimator for scoring the candidate graph networks. 

MMHC :
We use \cite{tsamardinos2006max} implementation of the MMHC Algorithm given in the bnlearn-R package \cite{scutari2012bnlearn}. The BIC criterion is employed as the scoring algorithm and we vary  the target nominal type I error rate of the conditional independence test for finding the best possible structure based on F-Score as the measure for correctness.

Gaussian Bayesian Network(GBN): 
We utilize the implementation of GBN given in \cite{cho2016reconstructing} where the conditional probability distribution (CPD) of each variable given the parents is defined to be a linear Gaussian distribution.The output of GBN based algorithm is the graph obtained by model averaging of the set of sampled graph structures drawn from the posterior distribution, where posterior represents how strong is each candidate graph structure to the underlying model given the data. Edge weights of the averaged, weighted resultant graph structure are normalized between 0 to 1 and thresholded at different levels to obtain different CPDAGs corresponding to each threshold level.

\textbf{Using mix of observation and intervention data}

GIES : 
We use \cite{hauser2012characterization} implementation given in pcalg-R for estimating markov equivalence of a DAG using GIES algorithm. $l$0-penalized Gaussian maximum likelihood estimator is used for scoring candidate causal graph structures learned jointly from interventional and observational data.

GBN : We use same implementation as discussed above for this case except that both observational and intervention data is used in this case.

\textbf{Assuming hidden variables:} We use FCI, FCI+ and RFCI algorithms implemented in pcalg-R for comparison across different datasets. For all three algorithms, we vary significance level from 0 to 1 in steps of 0.01 of conditional independence tests to obtain 100 CPDAGs for each algorithm and we choose the graph having best F-score measure.

\textbf{Assuming cycles:} We use CCD algorithm implemented in TETRAD \cite{spirtes2004tetrad} for learning cyclic causal structures. Causal structures corresponding to significance values varying between 0 to 1 with step-size of 0.1 are obtained and choose the graph with best F-score measure.

\textbf{Active Learning:} We explore the work of \cite{cho2016reconstructing} which uses active learning to priortize the interventions for optimal results using GBN framework. It learns the structure using top $n$ interventions out of all given interventions. We experimented on \textit{DREAM4$\_$10} dataset by setting the value of $n$ from 1 to 10 and then choosing the graph with maximum F-score.
% \subsection{Performance Metrics} 
% We compare the performance of algorithms using standard structure learning measures and using predictive accuracy by modeling the learned networks as causal bayesian networks.
% 
% \textbf{Structural efficiency based metrics:} \textit{F-score} and \textit{Area under ROC curve (AUC}) are used for measuring structural effectiveness of the algorithm. For the learned structure, each edge is defined as true positive, true negative, false positive, false negative based on the definitions in Figure~\ref{fig:confusion_matrix}. Structural precision, recall and false positive rate (FPR) are evaluated for varying thresholds on significance values/edge weights %using eq~\ref{eq:precision}, eq~\ref{eq:recall}, eq~\ref{eq:fpr} respectively.
% \begin{equation}
%   \small
%    Precision = \frac{\sum_{i} Tp_{i}}{\sum_{i} Tp_{i}+\sum_{i} Fp_{i}}
%    \label{eq:precision}
% \end{equation}
% \begin{equation}
%   \small
%    Recall = \frac{\sum_{i} Tp_{i}}{\sum_{i} Tp_{i}+\sum_{i} Fn_{i}}
%    \label{eq:recall}
% \end{equation}
% \begin{equation}
%   \small
%   FPR = \frac{\sum_{i} Fp_{i}}{\sum_{i} tn_{i}+\sum_{i} fp_{i}}
%    \label{eq:fpr}
% \end{equation}

% F-score is the harmonic mean of precision and recall and is computed at each threshold level. For this study, highest value of F-score is termed as \textit{structural F-score}. Area under ROC (curve plotting Recall versus fpr at different thresholds) is the desired AUC. %AUC signifies overall effectiveness of causal structure learning algorithm over different levels of parameters -significance value/edge weights.


% \textbf{Inferencing capability:} Standard metric for measuring performance of causal learning algorithms involve measures like structure hamming distance, F-score, count of missing and present edges. All these measures calculate structural efficiency of structure. However, practical need of causal structure learning involve applications require inferencing from the learned causal graph. Inferencing a causal network can assist in multiple practical applications involving predictions, intervention queries, counterfactual reasoning etc. Hence, we propose a measure called \textit{predictive accuracy}, which is used to measure the inferencing capability of the structure.% with best \textit{Structural F-score}.
% 
% In order to calculate predictive accuracy, we extend selected PAG/CPDAG to DAG using \cite{dor1992simple}. If no extension is possible, DAG corresponding to the skeleton of the PDAG is taken. Having obtained DAG structure of say $m$ variables, we model the DAG as causal Bayesian network with $m$ nodes. We predict the value of each node by observing the rest of $m-1$ nodes in a network using exact inferenec of Bayesian networks implemented in ~\cite{yadav2015business}. Further, we calculate normalized root mean squared error (NRMSE) of the predicted values with respect to the actual value in the data. Averaged out NRMSE across all nodes of each learned network is shown in Table \ref{NRMSE}.

\subsection{Comparison of algorithms based on performance metrics}

Table \ref{DREAM4-10} shows the Structural F-Score and AUC of fore mentioned causal structure learning algorithms for real datasets. Last row mentions the average calculated across all real datasets. It is seen that PC and GBN based structure learning algorithm outperform the remaining ones (all except active learning) in terms of both Structural F-score and AUC. 

Algorithms which utilize intervention data significantly perform better than their counterparts which use only observational data (GIES, GBN). Structural F-score and AUC for `Active learning' algorithm is shown in last column of Table \ref{DREAM4-10}. Prioritizing interventions using active learning framework leads to considerable increase of both the structural measures over rest of the algorithms.

\begin{table*}[]
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\textbf{Score}} & \multicolumn{11}{c|}{\textbf{Algorithms}} \\ \cline{3-13} 
 &  & \multicolumn{4}{c|}{On Observational Data} & \multicolumn{2}{c|}{On Intervention Data} & \multicolumn{3}{c|}{For Hidden Variables} & For cycles & \multirow{2}{*}{A.L} \\ \cline{3-12}
 &  & PC & GES & MMHC & GBN & GIES & GBN & FCI & FCI+ & RFCI & CCD &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_10\_1}} & \textit{F-Score} & 0.41 & 0.29 & 0.36 & 0.28 & 0.36 & 0.38 & 0.41 & 0.41 & 0.41 & 0.35 & 0.49 \\ \cline{2-13} 
 & \textit{AUC} & 0.55 & 0.59 & 0.54 & 0.56 & 0.64 & 0.67 & 0.27 & 0.34 & 0.34 & 0.53 & 0.71 \\ \cline{2-13} 
 & SHD & 15 & 18 & 11 & 29 & 17 & 22 & 11 & 14 & 16 &  &  \\ \cline{2-13} 
 & SID & 38 & 42 & 35 & 43 & 42 & 70 & 31 & 43 & 45 &  &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_10\_2}} & \textit{F-Score} & 0.45 & 0.28 & 0.34 & 0.37 & 0.29 & 0.44 & 0.42 & 0.44 & 0.44 & 0.42 & 0.45 \\ \cline{2-13} 
 & \textit{AUC} & 0.57 & 0.56 & 0.57 & 0.70 & 0.57 & 0.73 & 0.18 & 0.30 & 0.30 & 0.57 & 0.73 \\ \cline{2-13} 
 & SHD & 19 & 25 & 17 & 29 & 21 & 31 & 18 & 18 & 20 &  &  \\ \cline{2-13} 
 & SID & 65 & 56 & 57 & 44 & 51 & 60 & 69 & 47 & 69 &  &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_10\_3}} & \textit{F-Score} & 0.43 & 0.12 & 0.40 & 0.43 & 0.18 & 0.42 & 0.44 & 0.44 & 0.44 & 0.17 & 0.47 \\ \cline{2-13} 
 & \textit{AUC} & 0.54 & 0.46 & 0.61 & 0.68 & 0.50 & 0.67 & 0.27 & 0.33 & 0.33 & 0.47 & 0.74 \\ \cline{2-13} 
 & SHD & 14 & 24 & 11 & 24 & 24 & 21 & 16 & 18 & 17 &  &  \\ \cline{2-13} 
 & SID & 59 & 66 & 54 & 62 & 67 & 61 & 77 & 79 & 68 &  &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_10\_4}} & \textit{F-Score} & 0.32 & 0.12 & 0.27 & 0.34 & 0.29 & 0.75 & 0.30 & 0.32 & 0.32 & 0.44 & 0.62 \\ \cline{2-13} 
 & \textit{AUC} & 0.49 & 0.47 & 0.55 & 0.66 & 0.60 & 0.80 & 0.25 & 0.33 & 0.33 & 0.50 & 0.85 \\ \cline{2-13} 
 & SHD & 22 & 26 & 14 & 30 & 25 & 22 & 17 & 24 & 18 &  & 26 \\ \cline{2-13} 
 & SID & 75 & 59 & 63 & 71 & 59 & 65 & 70 & 56 & 69 &  & 72 \\ \hline
\multirow{4}{*}{\textit{DREAM4\_10\_5}} & \textit{F-Score} & 0.44 & 0.27 & 0.33 & 0.38 & 0.35 & 0.47 & 0.46 & 0.44 & 0.44 & 0.45 & 0.50 \\ \cline{2-13} 
 & \textit{AUC} & 0.65 & 0.60 & 0.57 & 0.73 & 0.66 & 0.83 & 0.32 & 0.38 & 0.38 & 0.58 & 0.83 \\ \cline{2-13} 
 & SHD & 9 & 20 & 12 & 20 & 20 & 18 & 11 & 11 & 11 &  & 22 \\ \cline{2-13} 
 & SID & 33 & 56 & 42 & 64 & 56 & 70 & 53 & 37 & 38 &  & 72 \\ \hline
\multirow{4}{*}{\textit{Sachs dataset}} & \textit{F-Score} & 0.45 & 0.28 & 0.41 & 0.36 & 0.10 & 0.15 & 0.45 & 0.47 & 0.45 & 0.45 & - \\ \cline{2-13} 
 & \textit{AUC} & 0.67 & 0.57 & 0.63 & 0.61 & 0.40 & 0.46 & 0.68 & 0.67 & 0.67 & 0.49 & - \\ \cline{2-13} 
 & SHD & 19 & 25 & 14 &  &  & 18 & 22 & 18 &  &  &  \\ \cline{2-13} 
 & SID & 98 & 85 & 77 &  &  & 78 & 88 & 79 &  &  &  \\ \hline
\multirow{4}{*}{\textit{\textbf{AVERAGE}}} & \textit{F-Score} & 0.42 & 0.23 & 0.35 & 0.36 & 0.26 & 0.44 & 0.41 & 0.42 & 0.42 & 0.38 & 0.50 \\ \cline{2-13} 
 & \textit{AUC} & 0.58 & 0.54 & 0.58 & 0.66 & 0.56 & 0.69 & 0.39 & 0.39 & 0.39 & 0.52 & 0.77 \\ \cline{2-13} 
 & SHD &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-13} 
 & SID &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
\caption{Table showing Structural F-Score and AUC for \textit{DREAM4$\_$10} and \textit{Sachs} datasets}
\label{DREAM4 10}
\end{table*}

%\vspace{-10pt}
\begin{table*}[]
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\textbf{SCORE}} & \multicolumn{6}{c|}{\textbf{Algorithms}} \\ \cline{3-8} 
 &  & \multicolumn{2}{c|}{On Observational Data} & On Intervention Data & \multicolumn{3}{c|}{For Hidden Variables} \\ \cline{3-8} 
 &  & PC & GES & GIES & FCI & FCI+ & RFCI \\ \hline
\multirow{4}{*}{\textit{DREAM4\_100\_1}} & \textit{F-Score} & 0.23 & 0.61 & 0.14 & 0.15 & 0.15 & 0.15 \\ \cline{2-8} 
 & \textit{AUC} & 0.58 & 0.57 & 0.58 & 0.18 & 0.31 & 0.31 \\ \cline{2-8} 
 & \textit{SHD} &  &  &  &  &  &  \\ \cline{2-8} 
 & \textit{SID} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_100\_2}} & \textit{F-Score} & 0.15 & 0.26 & 0.21 & 0.11 & 0.11 & 0.11 \\ \cline{2-8} 
 & \textit{AUC} & 0.008 & 0.58 & 0.55 & 0.002 & 0.002 & 0.002 \\ \cline{2-8} 
 & \textit{SHD} &  &  &  &  &  &  \\ \cline{2-8} 
 & \textit{SID} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_100\_3}} & \textit{F-Score} & 0.18 & 0.09 & 0.21 & 0.08 & 0.086 & 0.08 \\ \cline{2-8} 
 & \textit{AUC} & 0.01 & 0.49 & 0.55 & 0.002 & 0.002 & 0.002 \\ \cline{2-8} 
 & \textit{} &  &  &  &  &  &  \\ \cline{2-8} 
 & \textit{} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_100\_4}} & \textit{F-Score} & 0.17 & 0.09 & 0.07 & 0.17 & 0.174 & 0.17 \\ \cline{2-8} 
 & \textit{AUC} & 0.02 & 0.48 & 0.45 & 0.006 & 0.004 & 0.004 \\ \cline{2-8} 
 & \textit{SHD} &  &  &  &  &  &  \\ \cline{2-8} 
 & \textit{SID} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{\textit{DREAM4\_100\_5}} & \textit{F-Score} & 0.5 & 0.32 & 0.27 & 0.5 & 0.5 & 0.5 \\ \cline{2-8} 
 & \textit{AUC} & 0.05 & 0.63 & 0.60 & 0.030 & 0.03 & 0.03 \\ \cline{2-8} 
 & \textit{SHD} &  &  &  &  &  &  \\ \cline{2-8} 
 & \textit{SID} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{\textit{AVERAGE}} & \textit{F-Score} & 0.25 & 0.27 & 0.18 & 0.20 & 0.20 & 0.20 \\ \cline{2-8} 
 & \textit{AUC} & 0.17 & 0.55 & 0.55 & 0.05 & 0.07 & 0.07 \\ \cline{2-8} 
 & \textit{SHD} &  &  &  &  &  &  \\ \cline{2-8} 
 & \textit{SID} &  &  &  &  &  &  \\ \hline
\end{tabular}
\caption{Table showing structural F-score and AUC for \textit{DREAM4$\_$100 datasets}}
\label{DREAM4 100}
\end{table*}
%\vspace{-20pt}
Table \ref{DREAM4 100} shows structural performance of network having large number of nodes, 100 in this case. As evident from table \ref{DREAM4 100}, structural performance drops drastically in case of networks with higher number of nodes. Time taken for execution of structure learning exceeds 24 hour and inferencing algorithms crashes for large networks on Intel® Core™ i7-4600U CPU @ 2.10GHz × 4 system with 8gb RAM. Hence, current state of the art for causal structure learning algorithms does not work well for large node networks, present especially in biological domain. 

Table \ref{NRMSE} shows the averaged out NRMSE ($NRMSE_{av}$) across all nodes of each learned network. Last column of table \ref{NRMSE} shows the average of $NRMSE_{av}$ across all datasets. Lesser the $NRMSE_{av}$, better is the predictive accuracy. 

In terms of predictive accuracy, GES outperforms all other algorithms with $NRMSE_{av}$ of 8.845 followed by GBN learned on observation data and structure learning algorithms taking hidden nodes into account.

From table \ref{DREAM4-10} and \ref{NRMSE}, it is seen that algorithms having high structural F-score does not necessary have high inferencing capability. For eg, PC algorithm has high structural F-score but its predictive accuracy is low. This emphasizes that rather than just looking at traditional measures of finding structurally best causal network, inferencing capability of the learned causal structure should also be taken into account. Moreover, when true causal structure is not known, predictive accuracy can be used as an effective measure for finding the best causal structure. %This can also lead to the application of causal structure learning in practical fields requiring causal inferencing. 
   
\begin{table*}[ht]
\centering
\small
\begin{tabular}{|p{5.4em}|p{5.5em}|p{5.5em}|p{5.5em}|p{5.5em}|p{5.5em}|p{4.1em}|p{4.8em}|}
\hline
 \textit{Algorithm}& \textit{DREAM4$\_$10$\_$1} & \textit{DREAM4$\_$10$\_$2} & \textit{DREAM4$\_$10$\_$3} & \textit{DREAM4$\_$10$\_$4} & \textit{DREAM4$\_$10$\_$5} & \textit{Sachs} dataset & \textbf{AVERAGE} \\ \hline
PC                 & 9.01                       & 31.43                      & 32.79                      & 32.13                      & 33.15                      & 6.2       & 24.1183                   \\ \hline
GES               & 7.62                       & 8.3                        & 10.18                      & 10.43                      & 10.24                      & 6.3                  & \textbf{8.845}                     \\ \hline
GBN(obs)                    & $**$                         & 8.32                       & 11.57                      & 9.91                       & 11.17                      & 6.836                  & 9.56                   \\ \hline
MMHC                   & 16.84                        & 10.12                 & 22.39                    & 16.87                       & 12.58                      & 8.78                &                         14.59 \\ \hline
GIES              & 10.45                      & 11.3                       & 12.45                      & 11.67                      & 10.24                      & 7.32                    & 10.5716                   \\ \hline
GBN(obs+int)                & 17.54                      & 7.5                        & 17.5                       & 15.18                      & 23.52                      & 6.26                     & 14.58                         \\ \hline
FCI                & 15.72                      & 10.8                       & 10.04                      & 13.08                      & 14.66                      & 6.59                   & 11.815                    \\ \hline
FCIP             & 10.53                      & 11.05                      & 10.09                      & 7.82                       & 18.63                      & 6.24                   & 10.7267                   \\ \hline
RFCI              & 15.16                      & 7.76                       & 8.09                       & 7.87                       & 16.33                      & 6.39                  & 10.2667                   \\ \hline
Active Learning             & 12.27                      & 17.37                      & 15.58                      & 11.47                      & 11.97                      & $*$  & 13.73                                     \\ \hline
\end{tabular}
\caption{Averaged NRMSE, obs: (observational dataset) and int: (intervention dataset), ** took more than a day for execution (Results are not presented for the same). }
\label{NRMSE}

\end{table*}

Table \ref{Simulated dataset} compares the performances of causal structure learning algorithm applied on simulated dataset with respect to the performance of true causal structure. In this case, PC-algorithm outperforms all other algorithms both in terms of predictive accuracy and structural efficiency. Also, performance obtained by learned structure (PC) is very close to that of true graph.

True causal graphs for other datasets are cyclic in nature and hence throughout the analysis, we do not consider comparing predictive accuracy of other datasets with their true causal structures.

\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textit{\textbf{SCORE}}} & \multicolumn{5}{c|}{\textit{\textbf{Algorithms}}} \\ \cline{2-6} 
 & PC & \textit{GES} & \textit{FCI} & \textit{FCI+} & \textit{True graph} \\ \hline
F-score & 0.91 & 0.436 & 0.77 & 0.79 & 1 \\ \hline
AUC & 0.70 & 0.70 & 0.66 & 0.68 & 1 \\ \hline
SHD & 2 & 27 & 11 & 12 & 0 \\ \hline
SID & 12 & 33 & 65 & 71 & 0 \\ \hline
NRMSE & 7.44 & ** & 9.31 & 7.81 & 7.36 \\ \hline
\end{tabular}
\caption{Comparing performance measures on simulated dataset as compared to true structure. (**) representing algorithm took longer than 24 hours for execution}
\label{Simulated dataset}
\end{table}

We study the performances of causal structure learning algorithms based on the number of data samples in the dataset. \textit{DREAM4$\_$10} dataset is \textit{small-sized} dataset having less than 25 data samples whereas \textit{Simulated} dataset is \textit{large-sized} having greater than 10,000 samples. From Table \ref{Size comparison}, we observe that active learning based framework  having structural F-score of 0.50 and AUC of 0.77 shows best performance for \textit{small-sized} dataset while for \textit{large-sized} datasets, constraint based algorithms requiring only observation data performs well.

\begin{table}[]
\centering
\small
\label{Size comparison}
\begin{tabular}{|c|c|c|}
\hline
\multirow{2}{*}{Dataset size} & \multirow{2}{*}{$NRMSE_{av}$}  & Structural F-score \\ \cline{3-3}
                              &                             & AUC                \\ \hline
\multirow{2}{*}{Small-sized}  & \multirow{2}{*}{9.35 (GES)} & 0.50               \\ \cline{3-3}
                              &                             & 0.77               \\ \hline
\multirow{2}{*}{Large-sized}  & \multirow{2}{*}{7.44 (PC)} & 0.91              \\ \cline{3-3}
                              &                             & 0.7               \\ \hline                        
\end{tabular}
\caption{Comparison of performance metrics with respect to size of the datasets.}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{l|}{\textbf{Target Nodes}} \\ \cline{2-4} 
 & G1 & G5 & G10 \\ \hline
\textit{PC} &  &  &  \\ \hline
\textit{GES} &  &  &  \\ \hline
\textit{FCI} &  &  &  \\ \hline
\textit{FCI+} &  &  &  \\ \hline
\textit{RFCI} &  &  &  \\ \hline
\textit{MMHC} &  &  &  \\ \hline
\textit{Original Graph} &  &  &  \\ \hline
\end{tabular}
\caption{Change in target value as a percentage of the actual change on intervention(Delta) after performing counterfactual inference on different causal structure learning algorithms}
\label{Counterfactual}
\end{table} 
 
